Relativistic Spacecraft Propelled by Directed Energy

Achieving relativistic flight to enable extrasolar exploration is one of the dreams of humanity and the long term goal of our NASA Starlight program. We derive a fully relativistic solution for the motion of a spacecraft propelled by radiation pressure from a directed energy system. Depending on the system parameters, low mass spacecraft can achieve relativistic speeds; thereby enabling interstellar exploration. The diffraction of the directed energy system plays an important role and limits the maximum speed of the spacecraft. We consider 'photon recycling' as a possible method to achieving higher speeds. We also discuss recent claims that our previous work on this topic is incorrect and show that these claims arise from an improper treatment of causality.

==> relativisticrefs.tex <==
@article{marx1966interstellar,
  title={Interstellar vehicle propelled by terrestrial laser beam},
  author={Marx, George},
  journal={Nature},
  volume={211},
  year={1966},
  publisher={Roland Eoetvoes Univ., Budapest}
}

@article{einstein1905elektrodynamik,
  title={Zur elektrodynamik bewegter k{\"o}rper},
  author={Einstein, Albert},
  journal={Annalen der physik},
  volume={322},
  number={10},
  pages={891--921},
  year={1905},
  publisher={Wiley Online Library}
}


@article{PhysRev.21.483,
  title = {A Quantum Theory of the Scattering of X-rays by Light Elements},
  author = {Compton, Arthur H.},
  journal = {Phys. Rev.},
  volume = {21},
  issue = {5},
  pages = {483--502},
  numpages = {0},
  year = {1923},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.21.483},
  url = {https://link.aps.org/doi/10.1103/PhysRev.21.483}
}



@article{simmons1993marx,
	title={Was Marx right? or How efficient are laser driven interstellar spacecraft?},
	author={Simmons, JFL and McInnes, CR},
	journal={American journal of physics},
	volume={61},
	number={3},
	pages={205--207},
	year={1993},
	publisher={American Association of Physics Teachers}
}

@article{lubin2016roadmap,
  title={A Roadmap to Interstellar Flight},
  author={Lubin, Philip},
  journal={arXiv preprint arXiv:1604.01356},
  year={2016}
}

@article{redding1967interstellar,
  title={Interstellar vehicle propelled by terrestrial laser beam},
  author={Redding, JL},
  journal={Nature},
  volume={213},
  number={5076},
  pages={588--589},
  year={1967},
  publisher={Springer}
}


@inproceedings{hughes2013star,
  title={DE-STAR: phased-array laser technology for planetary defense and other scientific purposes},
  author={Hughes, Gary B and Lubin, Philip and Bible, Johanna and Bublitz, Jesse and Arriola, Josh and Motta, Caio and Suen, Jon and Johansson, Isabella and Riley, Jordan and Sarvian, Nilou and others},
  booktitle={SPIE Optical Engineering+ Applications},
  pages={88760J--88760J},
  year={2013},
  organization={International Society for Optics and Photonics}
}

@article{forward1984roundtrip,
  title={Roundtrip interstellar travel using laser-pushed lightsails},
  author={Forward, Robert L},
  journal={Journal of Spacecraft and Rockets},
  volume={21},
  number={2},
  pages={187--195},
  year={1984}
}

@article{bond1978project,
  title={Project Daedalus.},
  author={Bond, Alan and Martin, Anthony R},
  journal={Journal of the British Interplanetary Society},
  volume={31},
  pages={5},
  year={1978}
}

@article{beals1988project,
  title={Project Longshot: An Unmanned Probe to Alpha Centauri},
  author={Beals, Keith A and Beaulieu, Martin and Dembia, Frank J and Kerstiens, Joseph and Kramer, Daniel L and West, Jeffrey R and Zito, James A},
  year={1988}
}

@article{bae2012prospective,
  title={Prospective of photon propulsion for interstellar flight},
  author={Bae, Young K},
  journal={Physics Procedia},
  volume={38},
  pages={253--279},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{kosmo2015directed,
  title={Directed energy planetary defense},
  author={Kosmo, Kelly and Lubin, Philip and Hughes, Gary B and Griswold, Janelle and Zhang, Qicheng and Brashears, Travis},
  booktitle={2015 IEEE Aerospace Conference},
  pages={1--9},
  year={2015},
  organization={IEEE}
}


@article{lubin2015directed,
  title={Directed Energy for Planetary Defense and Exploration-Applications to Relativistic Propulsion and Interstellar and Intergalactic Communications},
  author={Lubin, PM and Hughes, GB and Bible, J and Johannson, I},
  journal={Journal of the British Interplanetary Society-JBIS},
  year={2015}
}

@article{bible2013relativistic,
  title={Relativistic propulsion using directed energy},
  author={Bible, Johanna and Johansson, Isabella and Hughes, Gary B and Lubin, Philip M},
  year={2013}
}

  	
@article{kipping,
  author={David Kipping},
  title={Relativistic Light Sails},
  journal={The Astronomical Journal},
  volume={153},
  number={6},
  pages={277},
  url={http://stacks.iop.org/1538-3881/153/i=6/a=277},
  year={2017},
  abstract={One proposed method for spacecraft to reach nearby stars is by accelerating sails using either solar radiation pressure or directed energy. This idea constitutes the thesis behind the Breakthrough Starshot project, which aims to accelerate a gram-mass spacecraft up to one-fifth the speed of light toward Proxima Centauri. For such a case, the combination of the sail’s low mass and relativistic velocity renders previous treatments incorrect at the 10% level, including that of Einstein himself in his seminal 1905 paper introducing special relativity. To address this, we present formulae for a sail’s acceleration, first in response to a single photon and then extended to an ensemble. We show how the sail’s motion in response to an ensemble of incident photons is equivalent to that of a single photon of energy equal to that of the ensemble. We use this principle of ensemble equivalence for both perfect and imperfect mirrors, enabling a simple analytic prediction of the sail’s velocity curve. Using our results and adopting putative parameters for Starshot , we estimate that previous relativistic treatments underestimate the spacecraft’s terminal velocity by ∼10% for the same incident energy. Additionally, we use a simple model to predict the sail’s temperature and diffraction beam losses during the laser firing period; this allows us to estimate that, for firing times of a few minutes and operating temperatures below 300°C (573 K), Starshot will require a sail that absorbs less than one in 260,000 photons.}
}
	
    
  @article{merali2016shooting,
  title={Shooting for a star},
  author={Merali, Zeeya},
  journal={Science},
  volume={352},
  number={6289},
  pages={1040--1041},
  year={2016},
  publisher={American Association for the Advancement of Science}
}


